Optimal Sharding for Scalable Blockchains with Deconstructed SMR

Sharding is proposed to enhance blockchain scalability. However, a size-security dilemma where every shard must be large enough to ensure its security constrains the efficacy of individual shards and the degree of sharding itself. Most existing sharding solutions therefore rely on either weakening the adversary or making stronger assumptions on network links. This paper presents Arete, an optimally scalable blockchain sharding protocol designed to resolve the dilemma based on an observation that if individual shards can tolerate a higher fraction of (Byzantine) faults, we can securely create smaller shards in a larger quantity. The key idea of Arete, therefore, is to improve the security resilience/threshold of shards by dividing the blockchain's State Machine Replication (SMR) process itself. Similar to modern blockchains, Arete first decouples SMR in three steps: transaction dissemination, ordering, and execution. However, unlike other blockchains, for Arete, a single ordering shard performs the ordering task while multiple processing shards perform the dissemination and execution of blocks. As processing shards do not run consensus, each of those can tolerate up to half compromised nodes. Moreover, the SMR process in the ordering shard is lightweight as it only operates on the block digests. Second, Arete considers safety and liveness against Byzantine failures separately to improve the safety threshold further while tolerating temporary liveness violations in a controlled manner. Apart from the creation of more optimal-size shards, such a deconstructed SMR scheme also empowers us to devise a novel certify-order-execute architecture to fully parallelize transaction handling, thereby improving the performance of sharding systems. We implement Arete and evaluate it on a AWS environment by running up to 500 nodes, showing that Arete outperforms the state-of-the-art sharding protocols.

==> analysis.tex <==
\section{Analysis}\label{section-analysis}
% Arete consists of multiple shards, each of which maintains a different ledger and can be viewed as an SMR. Typically, an SMR is required to ensure \textit{safety} where any two honest nodes store the same prefix ledger, and \textit{liveness} where all transactions are eventually finalized. However, in a sharding system, there exist cross-shard transactions involving multiple shards. The sharding system has to ensure each cross-shard transaction is finalized by all relevant shards consistently. To this end, we extend the definitions of safety and liveness of SMR to adapt to a sharding system.

% \begin{definition}[Sharding Safety]\label{def-system-safety}
%     The sharding safety requires: (i) any two honest nodes of the same shard maintain the same prefix ledger, and (ii) any two honest nodes from two different shards have the same finalization sequence and operation (commit or abort) for all cross-shard transactions involving the two shards.
% \end{definition}

% \begin{definition}[Sharding Liveness]\label{def-system-liveness}
%     Transactions sent to honest nodes are eventually finalized by their relevant shards.
% \end{definition}
This section proves Arete guarantees sharding safety and sharding liveness properties defined in \S~\ref{subsection-defnitions}. 

\subsection{Sharding Safety Analysis}
Since the ordering shard in Arete runs a BFT consensus to maintain its ledger, the inherent BFT consensus guarantees that nodes in the ordering shard maintain the same prefix ledger. Besides, cross-shard transactions only modify the states of processing shards but not the ordering shard. We therefore only discuss processing shards.
\begin{lemma}\label{lemma-intra-shard-safety}
    For every two honest nodes $N_i^{sid}$ and $N_j^{sid}$ with local ledgers $\mathfrak{L_i}^{sid}$ and $\mathfrak{L_j}^{sid}$ in processing shard $S_P^{sid}$, Arete guarantees: either $\mathfrak{L_i}^{sid} \subseteq \mathfrak{L_j}^{sid}$ or $\mathfrak{L_j}^{sid}\subseteq \mathfrak{L_i}^{sid}$.
\end{lemma}

\begin{myproof}{}
    For the sake of contradiction, assume there is a consensus round $r_c$ where $\mathfrak{L_i}^{sid}$ finalized a list of execution blocks with the digests $\mathit{EB_{dsts}}$, and $\mathfrak{L_j}^{sid}$ finalized another list of execution blocks with the digests $\mathit{EB'_{dsts}}$ ($\mathit{EB_{dsts}} \neq \mathit{EB'_{dsts}}$). However, since $\mathit{EB_{dsts}}$ and $\mathit{EB'_{dsts}}$ are the content of ordering blocks, it means the ordering shard finalizes two ordering blocks in $r_c$, violating the safety of the ordering shard, leading to a contradiction.
\end{myproof}

\begin{lemma}[Cross-shard Atomicity]\label{lemma-inter-shard-finalize}
    For any cross-shard transaction $\mathit{ctx}$ that is finalized by relevant processing shards, all relevant processing shards either commit or abort $\mathit{ctx}$.
\end{lemma}
\begin{myproof}{}
    Without loss of generality, we assume $\mathit{ctx}$ involves two processing shards $S_P^{m}$ and $S_P^{n}$. For the sake of contradiction, assume $S_P^{m}$ commits $\mathit{ctx}$ while $S_P^{n}$ aborts $\mathit{ctx}$. Recall from the COE model that the ordering shard picks all aggregators into its ordering blocks. Thus, $S_P^{m}$ receives an aggregator $\mathit{ARG}$ where $\mathit{ARG.vote}[\mathit{M_{ctx}}]=1$ while $S_P^{n}$ receives an aggregator $\mathit{ARG'}$ where $\mathit{ARG'.vote}[\mathit{M_{ctx}}]=0$, or there is another cross-shard transaction $\mathit{ctx'}$ conflicting with $\mathit{ctx}$ such that $\mathit{ARG.vote}[\mathit{M_{ctx'}}]=1$ and $\mathit{ARG'.vote}[\mathit{M_{ctx'}}]=0$. Both of them mean the ordering shard commits two different ordering blocks in the same round. However, the BFT consensus ensures the safety of the ordering shard, leading to a contradiction.
\end{myproof}

\begin{lemma}[Cross-shard Consistency]\label{lemma-inter-shard-order}
    For any two cross-shard transactions $\mathit{ctx_1}$ and $\mathit{ctx_2}$ that are finalized by relevant processing shards, either $\mathit{ctx_1}$ is finalized before $\mathit{ctx_2}$ or $\mathit{ctx_2}$ is finalized before $\mathit{ctx_1}$ in all relevant processing shards.
\end{lemma}
\begin{myproof}{}
    Without loss of generality, we assume $\mathit{ctx_1}$ and $\mathit{ctx_2}$ involve two processing shards $S_P^{m}$ and $S_P^{n}$. For the sake of contradiction, assume $S_P^{m}$ finalizes $\mathit{ctx_1}$ before $\mathit{ctx_2}$ while $S_P^{n}$ finalizes $\mathit{ctx_2}$ before $\mathit{ctx_1}$. 
    Recall from the \text{\footnotesize EXECUTE} stage that cross-shard transactions are finalized in the order of the $\mathit{VOTE}$ results of the aggregators. The above finalization results indicate that $S_P^{m}$ and $S_P^{n}$ receive different aggregators from the ordering shard, which violates the safety of the ordering shard and leads to a contradiction.
\end{myproof}

% \jianting{(maybe) prove Commitment-binding, i.e., each node can retrieve the same transactions with a commitment}

Lemma \ref{lemma-intra-shard-safety} proves Arete satisfies the condition(i) of Definition~\ref{def-system-safety}, and Lemmas \ref{lemma-inter-shard-finalize} and \ref{lemma-inter-shard-order} prove Arete satisfies the condition(ii) of Definition~\ref{def-system-safety}. Therefore, we have:

\begin{theorem}\label{theorem-system-safety}
    Arete guarantees the sharding safety.
\end{theorem}

\subsection{Sharding Liveness Analysis}

\begin{lemma}\label{lemma-liveness-order}
    Transactions sent to honest nodes are eventually ordered by the ordering shard. 
\end{lemma}
\begin{myproof}{}
    Recall from \S~\ref{subsection-system-architecture} that our shard reconfiguration mechanism ensures at least $f_S^{sid}\cdot |S_P^{sid}|+1$ nodes in each processing shard $S_P^{sid}$ eventually send their certificate blocks to the ordering shard. Since at most $f_S^{sid}$ fraction of nodes is Byzantine, the above condition ensures at least one honest node can certify new transactions to the ordering shard. Therefore, every transaction sent to honest nodes can be packed into a certificate block that will be eventually ordered by the ordering shard. 
    % Recall from \S~\ref{subsection-system-architecture} that our shard reconfiguration mechanism ensures the ratio of Byzantine nodes in each execution shard $S_P^{sid}$ is eventually no more than $f_L^{sid}$. When an honest node in $S_P^{sid}$ creates a certificate block $CB$, it can collect at least $(1-f_L^{sid})\cdot |S_P^{sid}|$ signatures for $CB$. Because of $f_S^{sid}+f_L^{sid} < 1$, we can conclude the honest node can collect at least $f_S^{sid}\cdot |S_P^{sid}|+1$ signatures for $CB$. Therefore, $CB$ is considered valid in the ordering shard (recall the validation condition discussed in the \text{\footnotesize ORDER} stage in \S~\ref{sec-coe-specification}). As the BFT consensus protocol provides the liveness for the ordering shard, the valid $CB$ will be eventually ordered by the ordering shard. In other words, transactions sent to the honest node creating $CB$ are eventually ordered by the ordering shard.
\end{myproof}

\begin{lemma}\label{lemma-liveness-availability}
    Honest nodes can obtain intact transactions for execution if these transactions have been ordered by the ordering shard.
\end{lemma}
\begin{myproof}{}
    \textcolor{blue}{If transactions are ordered by the ordering shard, it means their associated certificate blocks are valid (i.e., containing a quorum of signatures). From Lemma~\ref{lemma-data-availability}, we know that a valid certificate block enables nodes to retrieve all intact transactions corresponding with the block. Therefore, any honest node can eventually obtain these intact transactions.}
\end{myproof}

Lemmas \ref{lemma-liveness-order} and \ref{lemma-liveness-availability} jointly ensure each transaction sent to honest nodes can be handled by relevant processing shards and finalized eventually. Therefore, we have:
\begin{theorem}\label{theorem-system-liveness}
    Arete guarantees the sharding liveness.
\end{theorem}

==> applications.tex <==
\section{Application}\label{section-applications}
\jianting{Talk about the applications of our sharding scheme. (1) can be applied into non-sharded blockchains without weakening resilience to Byzantine failure or making network synchrony assumptions. (maybe we design a more general sharding scheme that can be extended by existing high-performance non-sharded SMR.) And our implementation was based on Hotstuff, which has been used by Diem as the core consensus.}

==> background.tex <==
\section{Related Work}
\label{appendix-related-work}
\noindent\textbf{Blockchain sharding}.
%Blockchain sharding has been proposed to scale blockchains by dividing nodes into multiple smaller shards such that these shards can process transactions in parallel with fewer resources. 
Many blockchain sharding works~\cite{Elastico, COSPLIT, redbelly} partition transaction executions/verification and require a final consensus broadcast to merge and update execution results for all nodes which still need to store the whole ledger without achieving the storage scalability. Subsequent works~\cite{chainspace, Omniledger, Rapidchain, Monoxide, ahl, hong2023prophet, harmony, xutwo} adopt a state-sharding scheme to partition the storage so that each node is only required to store a subset of the ledger. However, these sharding protocols require a large shard size to ensure system security as we analyzed in \S~\ref{section-problem}, which will limit the performance improvement that a sharding system can bring. 

To achieve smaller shard sizes, Instachain~\cite{ozdayi2022instachain}, \textsc{GearBox}~\cite{gearbox} and CoChain~\cite{licochain} allow the liveness or safety properties of a shard to be violated and introduce costly recovery mechanisms to resolve/recover unsecured shards. However, the high violation probability in these works makes them far away from practical usage. RIVET~\cite{rivet} proposes a reference-worker sharding framework like our work to reduce shard sizes by eliminating consensus from its worker shards. To alleviate the performance loss introduced by its reference-worker sharding framework, RIVET adopts an execute-order-commit architecture to process transactions. However, the execute-order-commit architecture has been shown to bring a high abortion rate of transactions due to its nondeterministic transaction order~\cite{sharma2019blurring,ruan2020transactional}.
Ethereum adopts a new data-sharding model (also referred to as Danksharding~\cite{danksharding}) where nodes in shards are only required to ensure the data availability rather than the validity of transactions. On a high level, Danksharding can reduce shard sizes by eliminating the honest majority assumption (e.g., $51\%$ honest assumption to ensure the validity of transactions and execution results). The data availability sampling (DAS) used by Danksharding allows a small set of honest nodes in each shard as long as these honest nodes can reconstruct the complete data (mainly consisting of transactions). The key to achieving this is that Danksharding relies on rollup technologies~\cite{optimisticrollup,zkrollup} to assist in executing transactions, where the validity of transaction executions is provided by layer-2 validators. However, offloading transaction executions into off-chain brings new challenges, such as interoperability across rollups, long transaction finality, and high computation cost.

Arete is designed to achieve practical shard sizes while keeping succinctness for a sharding protocol. In the meanwhile, the COE architecture adopted by Arete enhances the efficiency of handling cross-shard transactions, which is considered another major challenge in blockchain sharding. A research direction in blockchain sharding orthogonal to this paper is to reduce the number of cross-shard transactions~\cite{huang2022brokerchain, zhang2023txallo, optchain, krol2021shard, tao2020sharding}. Since these solutions are working on the account layer, such as strategically dividing accounts into different shards based on their dependencies, we emphasize that they are compatible with Arete to help reduce the number of cross-shard transactions.

% \bigbreak
\noindent\textbf{BFT protocols}. With rapid growth in adopting blockchain systems, BFT protocols have been studied extensively in the literature. Based on the network assumption, BFT protocols can be divided into three families: synchronous BFT~\cite{chan2020streamlet, abraham2020sync, pass2018thunderella}, partially synchronous BFT~\cite{pbft, gueta2019sbft, tendermint-bft, hotstuff, gelashvili2022jolteon}, and asynchronous BFT~\cite{miller2016honey, duan2018beat, guo2020dumbo, danezis2022narwhal, spiegelman2022bullshark, liu2023flexible}. These different BFT protocols have their inherent advantages and shortcomings. For instance, asynchronous BFT protocols remove the timing assumption and thus are more robust to a real-world network environment, but come with increased complexity, e.g., relying on randomness. It is worth noting that Arete can flexibly choose the BFT protocol for its ordering shard since the communications between execution shards and between the ordering shard and execution shards do not rely on any time-bound. Another major limitation of most BFT protocols is poor scalability, where the performance of the protocols cannot enhance well (or even decrease due to the increased communication complexity) with more nodes joining. Arete provides new insight into achieving a high-scalability BFT protocol.

\noindent\textbf{Parallel execution architecture in blockchains}. Apart from blockchain sharding protocols, many parallelized frameworks are implemented to enhance the performance of non-sharding blockchains. The main idea of these solutions is to decouple transaction execution and ordering. For instance, Hyperledger Fabric~\cite{hyperledger} proposes an execute-order-validate (EOV) architecture to support paralleling executions for transactions before ordering them. Nathan et al.~\cite{fabricssi} and BIDL~\cite{bidl} adopt an execute-order-parallel-validate (EOPV) that can hide the ordering cost by parallelizing the transaction execution and ordering. However, the executing-before/parallel-ordering architecture can incur read/write conflicts due to \textit{inconsistent access} to the same data, leading to the abortion of transactions and compromising performance. Many works~\cite{sharma2019blurring, ruan2020transactional} strive to reduce the abortion rate by applying some reordering algorithms but still suffer from a high abortion rate when the transaction workload involves frequent conflicts. In contrast, ACE~\cite{ACE} decouples transaction execution from consensus and offloads transactions into off-chain for parallelized execution after they are ordered. Many other works adopt a consensus/ordering-free parallelized framework for transaction execution. These solutions can eliminate the transaction abortion brought by the EOV architecture. However, they either rely on a single trusted server (e.g., NeuChain~\cite{neuchain}) or limit the applications built on their frameworks (e.g., FastPay~\cite{fastpay}, CryptoConcurrency~\cite{cryptoconcurrency}, and OrderlessChain~\cite{orderlesschain} exclusively support asset transfer).
Moreover, all the above parallelized solutions fail to capture a resource-intensive task in SMR (i.e., data dissemination) and cannot fully utilize bandwidth resources without parallelizing the data dissemination and ordering/execution. The data dissemination task has been pointed out as a main bottleneck in a high-performance SMR by recent works~\cite{prism, ohie}. Thus, the above parallelized solutions are poorly scalable. In contrast, the COE architecture used in Arete fully utilizes resources by parallelizing all the SMR tasks, and Arete shards the data dissemination and execution tasks for higher parallelism, making it highly scalable. Furthermore, different from the EOV architecture, the COE architecture realizes a deterministic global order before executing transactions. Thus, the transaction abortion rate in Arete is independent of the transaction workload and could be lower than that in the EOV architecture.

A line of Directed Acyclic Graph (DAG)-based consensus protocols~\cite{keidar2021all, danezis2022narwhal, spiegelman2022bullshark, shoal, suilutris, sailfish, kniep2024pilotfish} and its production blockchain Sui~\cite{sui} fully parallelize by separating data dissemination, ordering, and execution tasks as Arete. However, the DAG-based consensus protocols adopt a vertical scaling framework where newly joining nodes (also called \textit{workers}) must trust the primary node they associate, introducing a stronger trust assumption. In contrast, Arete adopts a horizontal scaling framework (i.e., sharding) without bringing new trust assumptions.





==> coe_old.tex <==
\section{The COE Model}\label{sec-coe-model}
In this section, we present the certify-order-execute (COE) model compatible with the ordering-execution sharding scheme to achieve scalability (\textbf{G3}), efficient cross-shard transactions commitment (\textbf{G4}), and high resource utilization (\textbf{G5}). We will first illustrate block structure in the COE model (for \textbf{G3}) and then demonstrate how ARETE can efficiently process transactions with the COE model (for \textbf{G4}). Finally, we propose an adaptive execution mechanism that is piggybacked on the COE model to achieve \textbf{G5}.

\subsection{Block Structure and Overview}\label{sec-coe-model-structure}
\textbf{Block structure}. The ordering-execution scheme in ARETE relies on one ordering shard to order all transactions from execution shards. To prevent the ordering shard from being a potential bottleneck, we revise the block structure in order to reduce computation, communication, and storage overheads for the ordering shard. Overall, there are three types of blocks in ARETE: execution block, certificate block, and ordering block.
% , as illustrated in Figure~\ref{fig:coe-model}(a). 
\begin{itemize}
    \item \textit{Execution blocks} are created and maintained by execution shards. An execution block ($EB_h^{sid}$ for short or) $EB=\langle state, sid, h, itxs\rangle_{\sigma_i}$ mainly consists of the latest state of the execution shard $state$, a list of locally ordered intra-shard transactions $itxs$, where $sid$ is the id of the execution shard $S_E^{sid}$, $h$ is the block height, and $\sigma_i$ is the signature of the block creator $i$.
    % The header of an execution block contains basic information about the block, such as shard ID, block height, and a hash of the previous block. A list of \textit{locally ordered intra-shard transactions} forms the body of an execution block. 
    % Note that the transaction order in an execution block is not the final order because the execution block has not yet been ordered by the ordering shard. 
    % The generation of execution blocks is leaderless, meaning that each node can create execution blocks, but only one execution block is picked for each block height by the ordering shard via consensus. The leaderless approach can guarantee liveness since execution shards have neither a consensus protocol nor a view-change mechanism to prevent Byzantine nodes from stopping to generate execution blocks.
    % \begin{equation}
    %     B_h^{sid, n}=(H_h, \{itxs\}, Sig_n).
    % \end{equation}
    \item \textit{Certificate blocks} are created to associate with execution blocks by execution shards. A certificate block ($CB_h^{sid}$ for short or) $CB=\langle sid, h, votes, d_{EB}, d_{ctxs}\rangle_{\sigma_{sid}}$ defines shard id, block height, a list of execution results for previous cross-shard transactions $vote$, a digest of its associated execution block $d_{EB}$, and a list of digests of cross-shard transactions $d_{ctxs}$. A valid certificate block must be certified by a quorum of nodes of $S_E^{sid}$ with their signatures $\sigma_{sid}$.
    
    % The header of a certificate block includes the hash of its associated execution block, shard ID, and block height. 
    % Different from the execution block using intra-shard transactions as its block body, the body of a certificate block is relevant to cross-shard transactions. This is because cross-shard transactions involve several execution shards and require coordination of the ordering shard. Specifically, the 
    % The body of a certificate block contains a \textit{vote set} $\{Votes\}$ for the cross-shard transactions from previous blocks and \textit{a list of new cross-shard transactions} $\{ctxs\}$ that will be ordered in the following block. 
    % We will demonstrate how these elements can help us to process cross-shard transactions in \S~\ref{sec-cross-tx-handle}. 
    % Furthermore, each certificate block must be signed by $(f_s+1)$ nodes in its execution shard.
    %, ensuring that at least one honest node recognizes the validity of the certificate block.
    % \begin{equation}
    %     C_h^{sid}=(H_h, \{votes\}, \{ctxs\}, Sigs).
    % \end{equation}
    \item \textit{Ordering blocks} are created by the ordering shard via its consensus protocol. An ordering block ($OB_h^{0}$ for short or) $OB=\langle h, \{d_{CB}\}_\Sigma, \{d_{ctxs}\}_\Sigma, \theta \rangle_{\sigma_{0}}$ consists of block height, a list of digests of certificate blocks from execution shards $\{d_{CB}\}_\Sigma$, a union of digests of globally ordered cross-shard transactions from execution shards $\{d_{ctxs}\}_\Sigma$, and an array $\theta$ that aggregates the voting results of cross-shard transactions in previous ordering blocks. Similarly, a valid ordering block must be certified by a quorum of nodes of the ordering shard $S_O$ with their signatures $\sigma_{0}$.
    
    % The ordering blocks are used to order transactions as well as coordinate cross-shard transactions. Therefore, an ordering block contains a $\{Arg\}$ that aggregates the voting results of cross-shard transactions in previous blocks, digests of certificate blocks $\{dgst\}$, a globally ordered list of cross-shard transactions $\{ctxs\}$, and a quorum certificate $QC$. 
    % Specifically, $\{Arg\}$ aggregates the voting results of cross-shard transactions in previous blocks (i.e., whether a cross-shard transaction is executed successfully by all relevant execution shards). $\{ctx\}$ contains cross-shard transactions that are from all execution shards in the current consensus round. Cross-shard transactions in the ordered $\{ctx\}$ will be processed by relevant execution shards in the next consensus round. $<Blocks>$ contains those certificate blocks that are chosen by the ordering shard and will be committed into ledgers of relevant execution shards. According to the chosen certificated blocks, nodes in the same execution shard can reach a consistent state.
    % \begin{equation}
    %     B_h^{0}=(H_h, \{Arg\}, \{dgst\}, \{ctxs\}, QC).
    % \end{equation}
\end{itemize}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=3.2in]{figure/transaction-process.pdf}
%     \caption{The block structures and workflow of the COE model.}
%     \label{fig:coe-model}
% \end{figure}

\textbf{Workflow of the COE model.} ARETE proceeds in rounds. Each round is associated with a height $h$ of an ordering block $OB_h^0$, where the ordering shard will run an instance of consensus to commit $OB_h^0$. A round is therefore called a \textit{consensus round}. The COE model consists of three stages: certifying blocks, ordering transactions, and executing transactions. 
% Assume the current consensus round is at $h$. 
Figure~\ref{fig:tx-process} shows the workflow of the COE model at two consecutive consensus rounds $h$ and $h+1$. 

In the first certifying stage, each node in an execution shard receives transactions from clients and packs intra-shard transactions into a new execution block. Next, the node creates a certificate block associated with the execution block. In particular, the node executes cross-shard transactions of previous order blocks to generate a vote set (see \S~\ref{sec-coe-tx-processing} for more details). The vote set along with a list of new cross-shard transactions is accumulated into the certificate block. The node then sends both the execution block and the certificate block to all nodes of the same execution shard. Other nodes will check if the certificate block is valid and then reply with their signatures. A node considers a received certificate block valid if it satisfies the following validation conditions:
\begin{itemize}
    \item \textbf{V1:} the node receives its associated execution block;
    \item \textbf{V2:} the vote set is consistent with its;
    \item \textbf{V3:} the certificate block is the first one received from the creator at the block height \jianting{not necessary}.
\end{itemize}
Once the creator receives $f_s\cdot m+1$ signatures from other nodes (where $m$ is the size of its execution shard), it sends the certificate block attached with these signatures to the ordering shard.

In the ordering stage, nodes in the ordering shard run a consensus instance to decide on transaction order and coordinate the commitment of cross-shard transactions. They check the validity of certificate blocks, interpret received certificate blocks, and pack valid certificate blocks into a new ordering block. Note that for each execution shard, at most one certificate block can be picked at each block height. This guarantees consistency of the ledger in an execution shard even though nodes in the execution shard do not run any consensus protocol. With the packed certificate blocks, a global order for both intra-shard and cross-shard transactions can be established with a pre-defined rule (we will discuss it in \S~\ref{sec-coe-tx-processing}). To coordinate the commitment of cross-shard transactions, nodes in the ordering shard aggregate the voting messages for those cross-shard transactions that have been ordered in previous ordering blocks. 
% Execution shards will commit or abort related cross-shard transactions according to the aggregation results.

In the final execution stage, execution shards execute and commit transactions based on the established transaction order along with the aggregation results in the committed ordering block. If a node has no complete transactions in its mempool due to the partially synchronous network or Byzantine behaviors, it will synchronize the missing transactions from other nodes. The $f_S\cdot m+1$ signatures in the certifying stage guarantee at least one honest node receives all transactions. Therefore, each honest node in execution shards is able to execute the ordered transactions.  
% Specifically, nodes in an execution shard first commit cross-shard transactions $\{ctx\}_{<h}$ on the aggregation messages $Arg$. Next, they execute and commit intra-shard transactions $\{itx\}_h$ associated with the chosen certificate block. Finally, they execute the cross-shard transactions $\{ctx\}_h$ ordered by the received ordering block. The execution results of $\{ctx\}_h$ will be used as the vote set of the next execution block. 
All nodes in the sharding system repeat the procedure of certify-order-execute to keep processing transactions.

\textbf{Achieving G3}. The COE model scales our sharding system in three aspects. First, since execution shards help verify transactions via the certifying stage, the ordering shard neither validates nor executes every transaction of the blocks, which reduces the computation overhead. Second, due to the separation of execution blocks and certificate blocks, intra-shard transactions are not delivered to the ordering shard, which reduces the communication overhead. Finally, since execution shards provide data availability for cross-shard transactions, the transaction data in the ordering shard can be pruned once they are committed, which reduces the storage overhead.

%\begin{algorithm}[t]
%% \label{alg-fairness-order}
%    \small
%    \caption{The COE model (for node in execution shard)}
%    \label{alg-order}
%    \begin{algorithmic}[1]
%        \Statex {\footnotesize \color{gray}$\blacktriangleright$  Step $1$: CrossLinks preparing}
%        \State \textbf{upon} receiving a CrossLink $S_i.CL$ from shard $S_i$ \textbf{do}
%            \State \hspace*{4mm} \textbf{if} {$S_i.CL.h = shardCLs[i].rear.h+1$} \textbf{then} \\\Comment{{\footnotesize \color{gray}$S_i.CL$ has a consecutive block height of the latest added CrossLink}}
%            \State \hspace*{8mm} $shardCLs[i]$ $\leftarrow add$ ($shardCLs[i]$, $S_i.CL$)
%            \\\Comment{{\footnotesize \color{gray} packs all CrossLinks with block heights that are consecutive with that of the last CrossLink in $shardCLs[i]$}}
%            \State \hspace*{8mm} \textbf{for all} {$CL \in CLPool$} \textbf{do}
%            \State \hspace*{12mm} \textbf{if} {$CL.h = shardCLs[i].rear.h+1$} \textbf{then}
%            \State \hspace*{16mm} $shardCLs[i]$ $\leftarrow add$ ($shardCLs[i]$, $CL$)
%            \State \hspace*{8mm} $shardLastTS[i]$ $\leftarrow$ $shardCLs[i].rear.blockTS$
%            \State \hspace*{4mm} \textbf{elseIf} {$S_i.CL.h > shardCLs[i].rear.h+1$} \textbf{then}  
%            \State \hspace*{8mm} add $S_i.CL$ to the CrossLink pool $CLPool$
%        
%        {\footnotesize \color{gray}\Statex $\blacktriangleright$ Step $2$: CrossLinks filtering}
%        \State \hspace*{4mm} \textbf{if} {$|shardCLs[i]|\geq 1, \forall 1 \leq i \leq m$} \textbf{then}
%        \State \hspace*{8mm} Choose all CrossLinks from $shardCLs$
%        with a block timestamp $blockTS \leq \min_{1 \leq i \leq m}\{shardLastTS[i]\}$.
%        
%        {\footnotesize \color{gray} \Statex $\blacktriangleright$ Step $3$: Transactions ordering}
%        \State \hspace*{4mm} \textbf{for each} {$CL$ chosen in $Step 2$} \textbf{do}
%            \State \hspace*{8mm} \textbf{for each} {$OTX \in CL$} \textbf{do}
%                \State \hspace*{12mm} \textbf{if} {$OTX$ call an OSC maintained by $S_i$} \textbf{then}
%                \State \hspace*{16mm} $CCLs[i]\leftarrow addWithOrder(CCLs[i], OTX)$
%
%    \end{algorithmic}
%\end{algorithm}

\subsection{Transaction Processing}\label{sec-coe-tx-processing}
\jianting{TODO: 1) don't wait for at least one. Use lock-based protocol. In this case, may lead to order-but-not-execute.
2) classify two types of cross-shard transaction: (i) cross-shard transfer: can be committed in one round; (ii) cross-shard state transaction: requires locks;}

Due to the separation of state, there are two kinds of transactions in ARETE: the \textit{intra-shard transaction} that involves data from one execution shard, and the \textit{cross-shard transaction} that involves data from several execution shards. As involving data from several shards, a cross-shard transaction will be divided into multiple \textit{intra-shard sub-transactions} which are then sent to relevant shards for collaborative execution. As mentioned in \S~\ref{subsection-model}, here we only consider exchange-free cross-shard transactions, where all relevant shards can handle the sub-transactions independently without exchanging data.

% Generally, cross-shard transactions can be classified into two types based on whether they involve state exchange when being handled. The first type, \textit{exchange-free} \jianting{should we change another name}, is the cross-shard transaction that all relevant shards can handle the sub-transactions independently without exchanging data with each other, such as a cross-shard transfer or the interactions of smart contracts within the same shard. The second type otherwise, \textit{state-exchange}, is the cross-shard transaction that some relevant shards rely on the data provided by other shards to execute their sub-transactions. 
% Stage-exchange cross-shard transactions only exist in smart contract interactions, i.e., a smart contract invokes other smart contracts during its execution. For instance, \jianting{give an example for state-exchange cross-shard transaction}. 
% We emphasize that state-exchange cross-shard transactions can be converted to exchange-free cross-shard transactions or be eliminated via some speculative execution mechanisms (see \S~\ref{sec-discussion} for more details). Therefore, in this paper, we focus on processing exchange-free cross-shard transactions. 

Similar to previous sharding systems, intra-shard transactions in ARETE can be committed within one consensus round. More importantly, exchange-free cross-shard transactions in ARETE can be processed more efficiently compared with previous sharding systems adopting a two-phase lock-based commit protocol. ARETE achieves the above assets via a \textit{deterministic global order} established by the ordering shard. The main idea is to strategically order intra-shard transactions and cross-shard transactions to eliminate data conflicts, as proved in many deterministic databases~\cite{thomson2012calvin,lu13aria,lin2021don}. Specifically, the ordering shard follows two ordering rules: (i) \textbf{R1}: \textit{all intra-shard transactions are ordered and executed before cross-shard transactions}; (ii) \textbf{R2}: \textit{transactions are committed in the order they are executed}. 

Figure~\ref{fig:tx-process} shows an overview of processing transactions across two consensus rounds $h$ and $h+1$. We assume these two consensus rounds cover intra-shard transactions $itx_1^1,itx_5^1$ from execution shard $S_E^1$ and $itx_2^2,itx_6^2$ from $S_E^2$, and exchange-free cross-shard transactions $ctx_3^{1,2},ctx_4^{1,2}$ relevant to $S_E^1$, $S_E^2$. Note that the transmission of intra-shard/cross-shard transactions between the ordering shard and execution shards is in the format of a digest. Here we neglect their formats for illustration purposes.
% For illustration purposes, we assume the following transactions:

\begin{figure*}[ht]
	\centering
	\includegraphics[width=6.5in]{figure/tx-process.pdf}
	\caption{Overview of processing transactions (\dashedarrow: messages, \solidarrow: hash links).}
	\label{fig:tx-process}
\end{figure*}

\begin{itemize}
    \item Steps 1.1 and 1.2 (Certifying stage in $h$): Nodes in $S_E^1$ create a certificate block $CB_h^1$ that certifies $itx_1^1$ and $ctx_3^{1,2}$. Similarly, a certificate block $CB_h^2$ that certifies $itx_2^2$ and $ctx_4^{1,2}$ is created by $S_E^2$. $CB_h^1$ and $CB_h^2$ are then sent to the ordering shard $S_O$ for consensus. 
    \item Step 2 (Ordering stage in $h$): Nodes in $S_O$ run an instance of consensus to order transactions associated with $CB_h^1$ and $CB_h^2$, outputting an ordering block $OB_h^0$. Based on our pre-defined ordering rule \textbf{R1}, intra-shard transactions are ordered before cross-shard transactions. The eventual global order of consensus round $h$ is $\{itx_1^1, itx_2^2, ctx_3^{1,2}, ctx_4^{1,2}\}$.
    \item Steps 3.1(2)a and 3.1(2)b (Execution stage in $h$): According to the transaction order defined in $OB_h^O$, $S_E^1$ first executes and commits $itx_1^1$ (step 3.1a). Then, $S_E^1$ executes $ctx_3^{1,2}$ and $ctx_4^{1,2}$, generating corresponding voting message $vote_3^1$ and $vote_4^1$ (step 3.1b). $vote_{txid}^{sid}$ represents the execution result of $ctx_{txid}$ on shard $S_E^{sid}$, i.e., success or failure. Similarly, $S_E^2$ commits its intra-shard transaction $itx_2^2$ and gets its voting messages $vote_3^2$ and $vote_4^2$. Note that since $ctx_3^{1,2}$ and $ctx_4^{1,2}$ are exchange-free cross-shard transactions, $S_E^1$ and $S_E^2$ can execute them independently.
    \item Steps 4.1 and 4.2 (Certifying stage in $h+1$): Nodes in $S_E^1$ (or, $S_E^2$) certify the voting messages $vote_3^1$ and $vote_4^1$ (or, $vote_3^2$ and $vote_4^2$) obtained from the last consensus round $h$. Additionally, new intra-shard transactions $itx_5^1$ and $itx_6^2$ can also be certified in this stage. The above certified transactions are then piggybacked by new certificate blocks $CB_{h+1}^1$ and $CB_{h+1}^2$ that are sent to $S_O$.
    \item Steps 5a and 5b (Ordering stage in $h+1$): Nodes in $S_O$ first aggregate the voting messages from $CB_{h+1}^1$ and $CB_{h+1}^2$ (Step 5a). Specifically, if both $vote_{txid}^1$ and $vote_{txid}^2$ (where $txid=3,4$) claim that $ctx_{txid}^{1,2}$ is executed successfully, then the aggregation $[vote]_{txid}$ indicates the cross-shard transaction $ctx_{txid}^{1,2}$ can be committed, or will be aborted otherwise. After aggregating, nodes in $S_O$ run an instance of consensus to order transactions associated with $CB_{h+1}^1$ and $CB_{h+1}^2$ (Step 5b), outputting an ordering block $OB_{h+1}^0$. Note that $ctx_3^{1,2}$ and $ctx_4^{1,2}$ are executed (in $h$) earlier than $itx_5^1$ and $itx_6^2$ (in $h+1$). Based on our pre-defined ordering rule \textbf{R2}, the final order of consensus round $h+1$ is $\{[vote]_3,[vote]_4,itx_5^1,itx_6^2\}$, where $[vote]_3$ and $[vote]_4$ represent $ctx_3^{1,2}$ and $ctx_4^{1,2}$, respectively.
    \item Steps 6.1(2)a and 6.1(2)b (Execution stage in $h+1$): In this stage, $S_E^1$ (or $S_E^2$) first commit $ctx_3^{1,2}$ and $ctx_4^{1,2}$ consistently according to the aggregations in $OB_{h+1}^0$ (Step 6.1a or Step 6.2a). Then, $S_E^1$ (or $S_E^2$) executes and commits the ordered intra-shard transaction $itx_5^1$ (or $itx_6^2$), as shown in Step 6.1a (6.2b) of Figure~\ref{fig:tx-process}.
\end{itemize}

% \textbf{Intra-shard transaction commitment}. Throughout the workflow depicted in Figure~\ref{fig:tx-process}. ARETE can commit intra-shard transactions within one consensus round. Specifically, $itx_1^1$ and $itx_2^2$ are committed in round $h$, while $itx_5^1$ and $itx_6^2$ are committed in round $h+1$.

% \textbf{Cross-shard transaction commitment}. ARETE can commit exchange-free cross-shard transactions at two consensus rounds without locking relevant states.

\jianting{After executing transactions, nodes in each execution shard send a signature on the commitment of the update state to others. Nodes keep $(f_S+1)$ signatures as the verifiable result.}

\textbf{Achieving G4}. Throughout the workflow depicted in Figure~\ref{fig:tx-process}, ARETE can commit cross-shard transactions $ctx_3^{1,2}$ and $ctx_4^{1,2}$ within two consecutive consensus rounds without locking relevant states. Additionally, ARETE can commit intra-shard transactions within one consensus round. 
Specifically, we achieve goal \textbf{G4} by the two ordering rules \textbf{R1} and \textbf{R2} defined in our deterministic global order.

% Overall, ARETE can efficiently commit intra-shard transactions and exchange-free cross-shard transactions by using a pre-defined ordering rule to establish a deterministic global order.


%\section{Adaptive Mempool Protocol}\label{sec-mempool-protocol}
\subsection{Adaptive Execution Protocol}\label{sec-adaptive-protocol}
% The COE model effectively solves the data conflict problems via its deterministic global order. Recall that to establish a deterministic global order, the ordering shard needs to wait for certificate blocks from \textit{all execution shards}. This works as a synchronization-ordering mechanism where each execution shard has the same block height. However, such a synchronization-ordering mechanism will lead to the performance of a sharding system is determined by the slowest execution shard. In a practical sharding system, different shards consisting of heterogeneous nodes will process transactions at various speeds. In this case, the whole system performance of the sharding system will be delayed by some slow execution shards. 
It is worth noting that to establish a deterministic global order, the ordering shard needs to wait for certificate blocks from all execution shards. It seems to deviate from the goal \textbf{G5} since a slow execution shard may generate a certificate block in a long time, and the ordering shard has to wait for this slow shard. To circumvent this issue, we present an \textit{adaptive execution protocol}. The main idea is to allow those fast execution shards to certify and eventually execute multiple blocks at one consensus round while achieving a deterministic global order for them. The adaptive execution protocol is designed as a complementary protocol that is integrated into the COE model. Figure \ref{sec-adaptive-protocol} presents an overview of the adaptive execution protocol, and we will detail it In the following.

\begin{figure}[t]
    \centering
    \includegraphics[width=3.0in]{figure/adaptive-execution.pdf}
    \caption{Adaptive execution protocol.}
    \label{fig:adp-exec}
\end{figure}

\textbf{Anchor blocks}. To enable an execution shard to certify multiple blocks at one consensus round, there must be one \textit{anchor block} in each execution shard at a consensus round. Specifically, when an execution shard certifies multiple blocks at a consensus round, \textit{the first certificate block} is recognized as the anchor block, e.g., $CB_{j+1}^2$ in Figure \ref{fig:adp-exec}. An anchor block is a certificate block with the functions we discussed in \S~\ref{sec-coe-model-structure}. It consists of a set of new cross-shard transactions, a quorum of signatures, and most importantly, a vote set for all cross-shard transactions from previous consensus rounds. The anchor blocks are used for the ordering shards to trace the heights of execution blocks in execution shards, as well as to aggregate the execution results for the two-phase commit protocol.

\textbf{Integration with the COE model}. The adaptive execution protocol allows an execution shard to continuously create execution blocks and certify them as certificate blocks before it is aware of a new ordering block. To integrate the adaptive execution protocol into the COE model, we need some minor modifications.

%The adaptive mempool protocol can be integrated into the COE model with minor modifications. 
First, a node in an execution shard is allowed to create and certify new blocks if and only if its created anchor block has been certified (i.e., received a quorum of signatures). Furthermore, along with the three validation conditions we mentioned in \S~\ref{sec-coe-model-structure} (\textbf{V1, V2, V3}), a node needs to check \textbf{V4:} it receives all the antecedent execution blocks and certificate blocks of a new certificate block before the node replies its signature on the new certificate block.

Second, nodes in the ordering shard need to maintain a table recording the height of the last certificate block that is committed for every execution shard. This prevents the ordering shard from picking outdated certificate blocks, i.e., blocks that have been committed. 

Third, when the ordering shard runs a consensus for execution shards, it needs to pick: (i) the vote set in the anchor block $CB_j^{sid}$; (ii) block header of one certificate block $CB_{j+n}^{sid}$; (iii) all cross-shard transaction sets in blocks from block height $j$ to $(j+n)$, for an execution shard $S_E^{sid}$. 

\textbf{Achieving G5}. With the adaptive execution protocol, ARETE supports executing multiple blocks of transactions in a fast execution shard within one consensus round. \jianting{talk more about it.}

==> discussion.tex <==
\section{Discussion}\label{sec-discussion}

\noindent\textcolor{red}{\textbf{The ordering shard as a potential bottleneck.} In Arete, there is only one ordering shard handling transactions from all processing shards (i.e., ordering transactions and coordinating cross-shard commitments). A fundamental concern for this design is that the ordering shard could become the bottleneck with more processing shards being created. An effective solution is to let processing shards create larger execution blocks, by which the size of data the ordering shard has to handle becomes smaller because processing shards create fewer certificate blocks. In other words, the overheads are amortized by processing shards. This solution is feasible with a reasonable incentive mechanism: 1) validators in processing shards can get more rewards (e.g., transaction fees) if execution blocks package more transactions; 2) the fees charged by the ordering shard of handling transactions for processing shards are set inversely proportional to the number of transactions included in execution blocks. Besides, we also present some optimizations to prevent the ordering shard from overwhelming overheads (cf. \S~\ref{appendix-discussion}).}

% \noindent \textbf{Complex cross-shard smart contracts}. In addition to one-shot cross-shard transactions, multi-shot cross-shard transactions may exist in a sharding system because of complex smart contracts that interact with each other and share their states during execution. When these complex smart contracts are deployed into a sharding system, it can lead to state exchanges between shards, introducing more complicated cross-shard coordination. In Arete, since there is a global order for transactions, execution shards can consistently synchronize all involved states and contract codes via off-chain communication so that each of them can execute multi-shot transactions independently. Such an off-chain synchronization solution for multi-shot cross-shard transactions can be integrated into the \text{\footnotesize{EXECUTE}} stage, but we leave this in our future work. In fact, how to efficiently and securely support complex cross-shard smart contracts is still an open problem for all existing sharding protocols. Instead, many works~\cite{rivet, tao2020sharding,krol2021shard} explore an alternative solution to eliminate complex cross-shard contracts, e.g., deploying contracts based on their dependencies by which there is no contract interaction cross shards. Furthermore, some speculation solutions~\cite{rivet, forerunner,hong2023prophet} are proposed to obtain involved states of contracts before executing them, by which shards are not required to exchange states. We emphasize that these solutions are compatible with Arete.

% \bigbreak
% \noindent \textbf{Leaderless cross-shard coordination.} Currently, Arete assigns the ordering shard to coordinate/lead the finalization of cross-shard transactions (\S~\ref{sec-coe-model-structure}). An alternative is to employ execution shards to communicate with each other directly to finalize cross-shard transactions, formulating a so-called \textit{leaderless coordination}. Specifically, instead of sending $\mathit{VOTE}$ results to the ordering shard, all execution shards need to broadcast their $\mathit{VOTE}$ results to the others. Then each execution shard can locally aggregate $\mathit{VOTE}$ results and finalize cross-shard transactions based on the established global order. However, this all-to-all communication brings significantly more communication overhead compared to the current leader-based cross-shard coordination.

% \bigbreak
% \noindent \textbf{Cascading abortion}. When Arete supports a lock-free execution, it can lead to a cascading abortion problem where aborting a cross-shard transaction $ctx$ will make all following cross-shard transactions conflicting with $ctx$ (i.e., involving in accessing the states modified by $ctx$) aborted, reducing performance. When the cascading abortion problem commonly exists in traditional distributed databases with an optimistic concurrency mechanism, we emphasize that there is a natural protection mechanism mitigating it in blockchain contexts. Specifically, the blockchain ledger asks every user to pay the transaction fees for its transaction execution. When a transaction is aborted, the user will not get the transaction fees back due to the failed execution. In our scenario, we can overcharge the transaction fees from a user who issues an aborted transaction. 
% \jianting{abort may outperform than lock-based solutions. Because locking is equal to not executing dependent transactions, and there always some hotspot contracts in a real-world blockchain network}
% This can reduce the cascading abortion attack where the adversary intentionally issues aborted transactions to compromise the system performance.

==> implementation.tex <==
\section{Implementation}\label{section-implementation}
We implement a prototype for ARETE in Rust, which uses Tokio\footnote{https://tokio.rs/} for asynchronous network, ed25519-dalek\footnote{https://github.com/dalek-cryptography/ed25519-dalek} for elliptic curve based signature, and RocksDB\footnote{https://rocksdb.org/} for persistent storage. The consensus protocol of the ordering shard adopts a variant of Hotstuff~\cite{gelashvili2022jolteon}. For the communications within each shard, we use TCP to realize reliable point-to-point channels. When a node sends a new message requiring signatures from other nodes of the same shard, it traces the reception of this message and keeps re-sending the message to which it did not receive an echo back. For communications between the ordering shard and execution shards, we allow nodes to randomly connect one or more nodes from the other shard. 
% Similar to works~\cite{gelashvili2022jolteon, danezis2022narwhal}, execution shards implement a batching technology to disseminate transactions. Specifically, nodes in execution shards first disseminate batches of transactions and then use hashes of batches to create execution blocks. The implementation involves around 6,500 lines of code. 
Our source codes of the implementation are public with the testing scripts \jianting{provide anonymous repository}.

We compare ARETE with GEARBOX~\cite{gearbox}, a state-of-the-art sharding protocol aiming to reduce the shard size. As discussed in \S~\ref{section-motivation}, GEARBOX separates safety and liveness properties. For a fair comparison, we evaluate this SOTA sharding protocol based on our codebase. However, as we show \S~\ref{section-problem}, the SOTA sharding protocol generates a different shard size $m^*$ compared to ARETE even under the same system parameters (i.e., same $n$, $s$, and $\lambda$). For instance, when setting $n=1,000$, $s=15\%$, and $\lambda=30$ and to guarantee $Pr[f_L]\geq 99.99\%$, we can get $m^*=90$, $f_S=39\%$ and $f_L=30\%$ for the SOTA sharding protocol (note that $f_S+2f_L<1$ here). It means nodes in the SOTA sharding protocol move to the next consensus stage until they receive $(1-f_L)\cdot m^*=63$ certificates from other nodes. In contrast, ARETE enables $m^*=32$, $f_S=61\%$ and $f_L=38\%$ under the same parameters and liveness probability (note that $f_S+f_L<1$ here), meaning nodes in execution shards of ARETE can move to the next stage with only $f_S\cdot m^*+1=20$ received certificates. Additionally, the SOTA sharding protocol adopts a two-phase commit protocol to handle cross-shard transactions, where any subsequent cross-shard transaction is blocked from accessing the same data until the previous cross-shard transaction is committed and releases the lock. Therefore, the goal of this comparison is to show how much improvement we can get by reducing shard size and the benefits of using our COE model to handle cross-shard transactions in a realistic network.

==> old-related.tex <==
\subsection{Blockchain Sharding Protocols}
\label{sec-related-work-sharding}
Sharding technology is first used in distributed systems for scalability by dividing the system into multiple smaller groups (a.k.a. shards) which can process transactions in parallel. Later, many works \cite{Elastico, Omniledger, Rapidchain} combined the sharding technology with blockchains to propose blockchain sharding. Different from traditional distributed sharding systems with the crashed model, blockchain sharding supports the Byzantine model where the Byzantine nodes can behave arbitrarily to violate the sharding protocol. There are three key components in a typical sharding system\footnote{For simplicity, we use sharding systems to represent blockchain sharding systems in the rest of this paper.}: Byzantine-resistant setup, intra-shard consensus, and cross-shard consensus.

\textbf{Byzantine-resistant setup}. Since a sharding system divides nodes into smaller consensus groups, it is easier for the adversary to control one group and thus compromise the security of the system. A sharding protocol needs to ensure each shard is controlled by the honest nodes at the beginning of shard formation. A straightforward-but-effective solution is to randomly assign nodes to different nodes so that attackers cannot selectively join in the same shard, and thus the solution prevents those attackers from controlling a shard. A common implementation of such a random assignment mechanism is PoW which requires each node to compute a PoW puzzle and the computation result will be used as the node's identity deciding which shard the node belongs to. Since the computation result is random, nodes will be randomly assigned to different shards.

\textbf{Intra-shard consensus}. In previous sharding systems, each shard needs to run an intra-shard consensus protocol to maintain its own blockchain. With the established identities in the system setup, a shard can use a Byzantine-fault tolerance (BFT) consensus protocol (more details are given in Section \ref{sec-related-work-bft}) as its intra-shard consensus. It is well-known that a BFT consensus protocol has a Byzantine threshold $f_{max}$ that measures how many Byzantine nodes the consensus group can have without violating the protocol security. Thus, once the ratio of Byzantine nodes in a shard exceeds $f_{max}$, the security of the shard is violated, in which Byzantine nodes can control the shard to return arbitrary outputs to users.

\textbf{Cross-shard consensus}. The two-phase commit protocol is widely used as the cross-shard consensus to process the cross-shard transaction that involves states maintained by multiple shards. The two-phase commit contains a voting phase and a commitment phase. In the voting phase, a cross-shard transaction is divided into several intra-shard transactions that are sent to relevant shards for processing. Each relevant shard runs a round of intra-shard consensus to execute the relevant intra-shard transaction, locking the modified states. In the commitment phase, each relevant shard will commit the modified states if it learns all relevant shards can execute the relevant intra-shard transactions successfully, and the cross-shard transaction is eventually committed. Since shards can still process other transactions during the cross-shard consensus, it is important to note that the traditional two-phase commit needs to lock the relevant states to prevent inconsistent state reads/writes.

\textbf{Limitations of previous sharding protocols}. The combination of Byzantine-resistant setup and BFT intra-shard consensus is not perfect. The former requires a large shard size that will limit the performance of the latter. In addition, the lock-based two-phase commit is low-efficiency since the lock mechanism limits the parallelism of handling conflicting transactions.

In this paper, we propose a new ordering-execution sharding scheme to reduce the shard size, while keeping as many original properties of blockchain sharding as possible (e.g., high-security level and excellent scalability). Interestingly, based on this sharding protocol, we propose a lock-free two-phase commit to efficiently handle cross-shard transactions. A previous work RIVET \cite{rivet} adopts a similar sharding scheme as ours, where it divides shards into one reference shard and multiple worker shards. However, different from ARETE which has a global order, RIVET only uses its reference shard to order cross-shard transactions and lets its worker shards optimistically execute intra-shard transactions. Without a global order before executing cross-shard and intra-shard transactions, the aborting rate of conflicting transactions will be high, which is not fully analyzed in the paper of RIVET. Besides, RIVET focuses on improving the efficiency of processing cross-shard transactions and lacks relevant discussions on how to form shards and what size a shard should be. Instead, we target reducing the shard size appropriately by our proposed ordering-execution sharding scheme and safety-liveness separation.

\textbf{RIVET} \textbf{1) different focusing problems; 2) although RIVET enhance cross-shard latency, but not good as ours since it adopts an execute-order-commit framework where no deterministic order exists. The optimistic/abort approach may increase more intra-shard latency.}

does not order intra-shard transactions in its reference shard. Instead, the reference shard only orders cross-shard transactions and \textit{state commitments} of worker shards. When worker shards \textit{optimistically} execute and generate commitment for intra-shard transactions, the reference shard may have an inconsistent commitment with worker shards. Note that RIVET orders cross-shard transactions after each latest commitment that a worker shard submits. The worker shard has to execute those cross-shard transactions before new intra-shard transactions; otherwise, the state commitment, generated by optimistic execution (i.e., execute intra-shard transactions before cross-shard transactions), is not accepted by the reference shard. This will lead to a rollback for intra-shard transactions in worker shards.

\subsection{SMR and BFT Consensus Protocols}
\label{sec-related-work-bft}
State Machine Replication (SMR) is a fundamental approach in distributed computing for building fault-tolerant systems. An SMR allows a group of nodes to maintain and reach a consistent state of the system by forcing the nodes to repeat the following tasks: transactions \emph{dissemination}, \emph{ordering}, and \emph{execution}. The core of the SMR is the consensus protocol, which defines a rule for the system nodes on how to agree on a consistent order that will be used for transactions' consistent execution. A blockchain is also a BFT-SMR (i.e., SMR in the Byzantine environment), which requires a BFT consensus protocol (such as PBFT \cite{pbft}, Hotstuff \cite{hotstuff}, and Tendermint \cite{tendermint}) to keep each node maintaining the same ledger. Typically, a blockchain needs to ensure the following security properties:
\begin{itemize}
    \item Safety. Any two honest nodes of the system store the same prefix ledger.
    \item Liveness. If a transaction is received by at least one honest node, then the transaction will be eventually handled and get a response from the system.
\end{itemize}

\noindent \textbf{BFT-SMR fault tolerance}. To guarantee the above properties, a BFT-SMR is subject to a Byzantine threshold $f_{max}$ which is used to measure the system's ability to ensure both safety and liveness. For example, in PBFT \cite{pbft} and Hotstuff \cite{hotstuff}, $f_{max}$ is equal to $1/3$, indicating that if the ratio of Byzantine nodes in the system $f < f_{max}$, then both safety and liveness can be guaranteed.

\noindent \textbf{Decoupling transaction execution from consensus.}

\noindent \textbf{Safety and liveness separation.} Many recent works \cite{malkhi2019flexible, momose2021multi, gearbox} propose to separate the safety and liveness properties so that a BFT-SMR can tolerate more Byzantine nodes when still guaranteeing one of the two properties. This comes with two separated Byzantine thresholds $f_S$ and $f_L$, which are used to represent the safety fault threshold and the liveness fault threshold respectively. Specifically, the BFT-SMR achieves safety in the presence of $f_S$ Byzantine nodes and liveness in the presence of $f_L$ Byzantine nodes. Therefore, when $f_S=f_L=f$, it can be considered that the BFT-SMR achieves both safety and liveness in the presence of $f$ Byzantine nodes, which is used in traditional BFT-SMR systems.

Separating safety and liveness enables a BFT-SMR to integrate with characteristic BFT consensus protocols. In many scenarios, safety is considered more important than liveness (this is consistent with the target of the partial synchrony model where safety is always satisfied yet liveness is achieved only under good network conditions). It can be proved that a BFT-SMR can guarantee safety as long as $f_S+2f_L < 1$ (see Section ? for more details). Therefore, a BFT-SMR can improve $f_S$ by reducing $f_L$ to tolerate more Byzantine nodes without compromising safety. In a blockchain sharding scenario, a higher $f_S$ can bring a smaller shard size, which will significantly reduce the consensus overhead for a shard and make the sharding system more practical. 

In this paper, we also utilize the idea derived from safety-liveness separation for the execution shard. However, different from previous safety-liveness separation protocols, ours is not built on a BFT-SMR since an execution shard does not run a consensus protocol. This brings a significant benefit to slimming shard size. Specifically, instead of $f_S+2f_L < 1$, an execution shard only needs $f_S+f_L < 1$ to achieve safety. This will make our sharding protocol more attractive in a practical scenario. We will give more details in Section ?.

% refer to \cite{momose2021multi}: This higher safety under synchrony can be very useful as it helps disincentivize rational players from attacking the system. If they do not have control over the network infrastructure, they would need to persuade a very large fraction of nodes to collude with them in order to succeed in breaking safety.

\subsection{Deterministic Execution in Distributed Database}\label{sec-related-work-deterministic}

==> processtxs.tex <==
\section{Transaction Processing in ARETE}\label{sec-tx-process}
In this section, we will present how ARETE handles transactions under the ordering-execution sharding scheme.
We first propose a \textit{certify-order-execute} model. This model incorporates the feature of ordering-execution separation to reduce communication overheads between the ordering shard and execution shards. More importantly, it prevents some potential attacks introduced by the ordering-execution separation in ARETE. Then, we depict the workflow of processing intra-shard transactions and finally demonstrate how ARETE handles cross-shard transactions harmoniously with intra-shard transactions.
% , where we propose a new cross-shard commit protocol, called \textit{lock-free two-phase commit protocol}. This new cross-shard commit protocol allows ARETE to eliminate the lock operation such that the system is able to continuously process conflicting transactions without being blocked. 

\begin{figure}[h]
    \centering
    \includegraphics[width=3.2in]{figure/transaction-process.pdf}
    \caption{Caption}
    \label{fig:tx-proccess}
\end{figure}

\subsection{The COE Model}
% \label{sec-COE-model}
In ARETE, we separate transaction ordering and execution. The ordering shard is only responsible for ordering transactions. Executing transactions, along with storing state data that is generated by transaction execution, is however completed by relevant execution shards. In this case, the ordering shard is not able to verify transactions and thus relies on execution shards to certify transactions before ordering them. To achieve this, we incorporate a new transaction processing model, called certify-order-execute (COE), into our ordering-execution separation framework. An illustration of the COE model can be seen in Figure \ref{fig:tx-proccess}. We first introduce block structures used in ARETE.

\noindent \textbf{Block structure}. In ARETE, the ordering shard and execution shards maintain different block structures according to their roles in the sharding system. For different functional needs, we decouple a block of the execution shard into two blocks: the execution block and the certificate block. Such a block decoupling enables us to optimize the efficiency of processing transactions and prevent some potential malicious behaviors, which will be discussed at the end of this section. Overall, there are three types of blocks in ARETE: execution block, certificate block, and ordering block. 
\begin{itemize}
    \item \textit{Execution blocks} are created and maintained by execution shards. The header of an execution block contains basic information about the block, such as shard ID, block height, and a hash of the previous block. A list of \textit{ordered intra-shard transactions} forms the body of an execution block. Note that the transaction order in an execution block is not the final order because the execution block has not yet been ordered by the ordering shard. The generation of execution blocks is leaderless, meaning that each node can create execution blocks, but only one execution block is picked for each block height by the ordering shard via consensus. The leaderless approach can guarantee liveness since execution shards have neither a consensus protocol nor a view-change mechanism to prevent Byzantine nodes from stopping to generate execution blocks.
    \item \textit{Certificate blocks} are created to associate with execution blocks. The header of a certificate block includes the hash of its associated execution block, shard ID, and block height. Different from the execution block using intra-shard transactions as its block body, the body of a certificate block are relevant to cross-shard transactions. This is because cross-shard transactions involve several execution shards and require coordination of the ordering shard. Specifically, the body of a certificate block contains a \textit{vote set} $\{Votes\}$ for the cross-shard transactions from previous blocks and \textit{a list of new cross-shard transactions} $\{ctxs\}$ that will be ordered in the following block. We will demonstrate how these elements can help us to process cross-shard transactions in \S~\ref{sec-cross-tx-handle}. Furthermore, each certificate block must be signed by $(f_s+1)$ nodes in its execution shard, ensuring that at least one honest node recognizes the validity of the certificate block.
    \item \textit{Ordering blocks} are created by the ordering shard via its consensus protocol. The ordering blocks are used to order transactions as well as coordinate cross-shard transactions. Therefore, an ordering block contains a list of aggregation $\{Arg\}$, an ordered list of cross-shard transactions $\{ctxs\}$, and a list of certificate blocks $<Blocks>$. Specifically, $\{Arg\}$ aggregates the voting results of cross-shard transactions in previous blocks (i.e., whether a cross-shard transaction is executed successfully by all relevant execution shards). $\{ctx\}$ contains cross-shard transactions that are from all execution shards in the current consensus round. Cross-shard transactions in the ordered $\{ctx\}$ will be processed by relevant execution shards in the next consensus round. $<Blocks>$ contains those certificate blocks that are chosen by the ordering shard and will be committed into ledgers of relevant execution shards. According to the chosen certificated blocks, nodes in the same execution shard can reach a consistent state.
\end{itemize}


\noindent \textbf{Workflow of COE model.} The COE model consists of three stages: certifying blocks, ordering transactions, and executing transactions. Assume both the ordering shard and execution shards are creating blocks at height $h$. In the first certifying stage, each node in an execution shard receives transactions from clients and packs intra-shard transactions $\{itx\}_h$ into a new execution block. Next, the node creates a certificate block associated with the execution block. In particular, the node executes cross-shard transactions of previous order blocks to generate a vote set (see \S~\ref{sec-cross-tx-handle} for more details). The vote set along with a list of new cross-shard transactions is accumulated into the certificate block. The node then broadcasts both the execution block and the certificate block it creates to ensure integrity and availability of the blocks. Other nodes in the same execution shards will check if the certificate block is valid and then reply with their signatures. A node considers a received certificate block valid if it satisfies the following validation conditions:
\begin{itemize}
    \item \textbf{V1:} the node receives its associated execution block;
    \item \textbf{V2:} the vote set is correct;
    \item \textbf{V3:} the certificate block is the first one received from the creator at the block height.
\end{itemize}
Once the creator receives $f_s+1$ signatures from other nodes, it sends the certificate block attached with these signatures to the ordering shard.

In the ordering stage, nodes in the ordering shard run a consensus instance to decide on transaction order and coordinate the commitment of cross-shard transactions. They check the validity of certificate blocks, interpret received certificate blocks, and pack valid certificate blocks into a new ordering block. Note that for each execution shard, at most one certificate block can be picked at each block height. This guarantees consistency of the ledger in an execution shard even though nodes in the execution shard do not run any consensus protocol. With the packed certificate blocks, a global order for both intra-shard and cross-shard transactions can be established with a pre-defined rule (we will discuss it in \S~\ref{sec-intra-tx-handle} and \S~\ref{sec-cross-tx-handle}). To coordinate the commitment of cross-shard transactions, nodes in the ordering shard aggregate the voting messages for those cross-shard transactions that have been ordered in previous ordering blocks. Execution shards will commit or abort related cross-shard transactions according to the aggregation results.

After an ordering block is committed, execution shards execute and commit transactions based on the established transaction order in the execution stage. Specifically, nodes in an execution shard first commit cross-shard transactions $\{ctx\}_{<h}$ on the aggregation messages $Arg$. Next, they execute and commit intra-shard transactions $\{itx\}_h$ associated with the chosen certificate block. Finally, they execute the cross-shard transactions $\{ctx\}_h$ ordered by the received ordering block. The execution results of $\{ctx\}_h$ will be used as the vote set of the next execution block. Nodes in the sharding system repeat the procedure of certify-order-execute to keep processing transactions.

\noindent \textbf{Conflicts resolution}. The COE model works round-by-round. Each round is associated with a block height $h$. The ordering shard runs an instance of consensus for each round to commit an ordering block. Therefore, a round of the COE model is also called a \textit{consensus round}. In a nutshell, the COE model circumvents data conflicts between intra-shard and cross-shard transactions (as mentioned in \textbf{C1}) by establishing a \textit{deterministic global order} for these transactions. In the following sections, we will show how we can utilize such a deterministic order to effectively commit both intra-shard and cross-shard transactions.

\jianting{Non-deterministic: cross-shard transactions can influence execution shards, invalidating their intra-shard transactions.}

%\begin{algorithm}[t]
%% \label{alg-fairness-order}
%    \small
%    \caption{The COE model (for node in execution shard)}
%    \label{alg-order}
%    \begin{algorithmic}[1]
%        \Statex {\footnotesize \color{gray}$\blacktriangleright$  Step $1$: CrossLinks preparing}
%        \State \textbf{upon} receiving a CrossLink $S_i.CL$ from shard $S_i$ \textbf{do}
%            \State \hspace*{4mm} \textbf{if} {$S_i.CL.h = shardCLs[i].rear.h+1$} \textbf{then} \\\Comment{{\footnotesize \color{gray}$S_i.CL$ has a consecutive block height of the latest added CrossLink}}
%            \State \hspace*{8mm} $shardCLs[i]$ $\leftarrow add$ ($shardCLs[i]$, $S_i.CL$)
%            \\\Comment{{\footnotesize \color{gray} packs all CrossLinks with block heights that are consecutive with that of the last CrossLink in $shardCLs[i]$}}
%            \State \hspace*{8mm} \textbf{for all} {$CL \in CLPool$} \textbf{do}
%            \State \hspace*{12mm} \textbf{if} {$CL.h = shardCLs[i].rear.h+1$} \textbf{then}
%            \State \hspace*{16mm} $shardCLs[i]$ $\leftarrow add$ ($shardCLs[i]$, $CL$)
%            \State \hspace*{8mm} $shardLastTS[i]$ $\leftarrow$ $shardCLs[i].rear.blockTS$
%            \State \hspace*{4mm} \textbf{elseIf} {$S_i.CL.h > shardCLs[i].rear.h+1$} \textbf{then}  
%            \State \hspace*{8mm} add $S_i.CL$ to the CrossLink pool $CLPool$
%        
%        {\footnotesize \color{gray}\Statex $\blacktriangleright$ Step $2$: CrossLinks filtering}
%        \State \hspace*{4mm} \textbf{if} {$|shardCLs[i]|\geq 1, \forall 1 \leq i \leq m$} \textbf{then}
%        \State \hspace*{8mm} Choose all CrossLinks from $shardCLs$
%        with a block timestamp $blockTS \leq \min_{1 \leq i \leq m}\{shardLastTS[i]\}$.
%        
%        {\footnotesize \color{gray} \Statex $\blacktriangleright$ Step $3$: Transactions ordering}
%        \State \hspace*{4mm} \textbf{for each} {$CL$ chosen in $Step 2$} \textbf{do}
%            \State \hspace*{8mm} \textbf{for each} {$OTX \in CL$} \textbf{do}
%                \State \hspace*{12mm} \textbf{if} {$OTX$ call an OSC maintained by $S_i$} \textbf{then}
%                \State \hspace*{16mm} $CCLs[i]\leftarrow addWithOrder(CCLs[i], OTX)$
%
%    \end{algorithmic}
%\end{algorithm}

\subsection{Intra-shard Transaction Processing}\label{sec-intra-tx-handle}
Intra-shard transactions can be affected by cross-shard transactions when the latter has data contention with the former, e.g., both of them access the same state. Specifically, processing a cross-shard transaction inevitably generates an \textit{intermediate state}, i.e., a state that an execution shard modifies but does not commit it before all relevant execution shards agree to commit the transaction. These intermediate states cannot be accessed by intra-shard transactions as it involves dirty reads/writes, leading to inconsistency. Previous sharding systems resolve this data conflict by locking intermediate states and not ordering conflicting intra-shard transactions after them when a shard performs intra-shard consensus. However, in our ordering-execution sharding framework, it will become more challenging because execution shards neither run intra-shard consensus nor order transactions independently. An unpredictable global order may lead to the failure of executing and committing intra-shard transactions, sacrificing the system performance.

In ARETE, a deterministic global order can prevent execution shards from accessing these intermediate states, allowing intra-shard transactions to be committed effectively.
%However, with a deterministic global order, an execution shard is immune to the modified but uncommitted state. 
An illustrative example of processing intra-shard transactions is shown in Figure \ref{fig:tx-proccess}(b).

\begin{itemize}
    \item Steps 1a and 1b: At the beginning of a consensus round $h$, a node of an execution shard $S_E^i$ randomly packs intra-shard transactions $\{itxs\}_h^i$ from its mempool to form an execution block $B_h^i$. $B_h^i$ will be associated with a certificate block $C_h^i$, which will be sent to the ordering shard for consensus. 
    \item Steps 2a: Nodes $\mathcal{N}$ in the ordering shard can receive multiple certificate blocks that are created by different nodes from an execution shard, and receive certificate blocks from different execution shards. However, $\mathcal{N}$ only picks one certificate block from each execution shard for consensus. More importantly, in the new ordering block $B_h^O$, all intra-shard transactions $\{itxs\}_h$ will be ordered before cross-shard transactions $\{ctx\}_h$.
    \item Step 3b: Each execution shard now can execute and commit intra-shard transactions based on the transaction order in $B_h^O$. 
\end{itemize}

Such a deterministic global order ensures that all intra-shard transactions are ordered before and do not access to any intermediate states generated by cross-shard transactions from the same consensus height. As a consequence, the COE model prevent data conflicts.

\subsection{Cross-shard Transaction Processing}\label{sec-cross-tx-handle}
In a blockchain sharding system, a cross-shard transaction is defined as a transaction that involves data from several shards. As shards can only modify and update the data they maintain, a cross-shard transaction will be divided into multiple \textit{intra-shard sub-transactions} which are then sent to relevant shards for handling. Generally, cross-shard transactions can be classified into two types based on whether they involve state exchange when being handled. The first type, \textit{exchange-free}, is the cross-shard transaction that all relevant shards can handle the sub-transactions independently without exchanging data with each other, e.g., a cross-shard transfer. The second type, \textit{state-exchange}, is the cross-shard transaction that some relevant shards rely on the data provided by other shards to execute their sub-transactions. For instance, \jianting{give an example for state-exchange cross-shard transaction}. 

Based on the types of cross-shard transactions, ARETE handles cross-shard transactions in different ways with the COE model. Specifically, we adopt 1) a lock-free commit mechanism for exchange-free cross-shard transactions; 2) a lock-based commit mechanism for state-exchange cross-shard transactions.

\begin{figure}[h]
	\centering
	\includegraphics[width=3.3in]{figure/lock-free-commit.pdf}
	\caption{Adaptive mempool protocol}
	\label{fig:lock-free-commit}
\end{figure}

\textbf{1) Lock-free commit.} With a deterministic global order provided by the COE model, exchange-free cross-shard transactions can be committed in two phases without locking any relevant data. Figure \ref{fig:lock-free-commit} illustrates an example of handling exchange-free transactions. Assume at consensus round $h$, a set of cross-shard transactions $<ctxs>_h^1$ from execution shard $S_E^1$ is going to be handled. Without loss of generality, we assume $S_E^1$ and $S_E^2$ are the two execution shards relevant to $<ctxs>_h^1$. The lock-free commit protocol commits $<ctxs>_h^1$ in the vote phase and commit phase:

\noindent \textbf{Vote phase:} In this phase, relevant execution shards execute cross-shard transactions locally.

\begin{itemize}
	\item Step 1: Nodes in $S_E^1$ create a certificate block $c_h^1$ that certifies $<ctxs>_h^1$ along with a new set of intra-shard transactions $\{itxs\}_h^1$. $c_h^1$ is then sent to the ordering shard $S_O$ for consensus.
	\item Step 2: Nodes in $S_O$ run an instance of consensus that picks $c_h^1$ as the only certificate block of $S_E^1$ at height $h$.
	\item Steps 3a-3b: According to the deterministic global order, all execution shards first execute and commit their intra-shard transactions at height $h$ (step 3a). After that, the relevant execution shards $S_E^1$ and $S_E^2$ execute $<ctxs>_h^1$ (step 3b). As no state exchange is involved, $S_E^1$ and $S_E^2$ can complete this process independently. Eventually, both $S_E^1$ and $S_E^2$ derive their respective vote set $\{Vote\}_h^1$ and $\{Vote\}_h^2$. Specifically, $\{Vote\}_h$ records a map from cross-shard transactions to execution results. For example, a transaction $CTX_1$ that is executed successfully in $S_E^1$ will be associated with $\{Vote\}_h^1[CTX_1]=S$, or $\{Vote\}_h^1[CTX_1]=F$ if it is failed.
\end{itemize}

\noindent \textbf{Commit phase:} In this phase, relevant execution shards commit cross-shard transactions based on the vote sets from the vote phase.

\begin{itemize}
	\item Step 4: Nodes in $S_E^1$ create a new certificate block $c_{h+1}^1$ that certifies $\{Vote\}_h^1$, new transactions $\{itxs\}_{h+1}^1$ and $c_{h+1}^1$.
	\item Step 5: $S_O$ aggregate the execution results for $c_h^1$ from $\{Vote\}_h^1$ and $\{Vote\}_h^2$. Nodes in $S_O$ run an instance of consensus to create an ordering block $B_{h+1}^O$ that picks certificate blocks from $S_E^1$ and $S_E^2$ at height $h+1$.
	\item Steps 6a and 6b: According to the aggregations in $B_{h+1}^O$, $S_E^1$ and $S_E^2$ commit $c_h^1$ consistently (step 6a). Specifically, if a transaction $CTX_1$ is executed successfully in both $S_E^1$ and $S_E^2$, i.e., $\{Vote\}_h^1[CTX_1]=S$ $\{Vote\}_h^2[CTX_1]=S$, then $CTX_1$ is committed by both $S_E^1$ and $S_E^2$, or is aborted otherwise.
\end{itemize}

%packs a set of cross-shard transactions $<ctxs>_h^1$, along with intra-shard transactions $\{itxs\}_h^1$, into a certificate block $C_h^1$.

\textbf{2) Lock-based commit.}

%Cross-shard transactions are notorious in sharding systems because they involve multiple shards' state data and introduce a cost coordination mechanism that will \textit{lock} relevant data during their processing, a.k.a. lock-based two-phase commit protocol. With the global ordering property given by our ordering-execution sharding framework, we propose a new lock-free two-phase commit protocol.


\noindent \textbf{Optimization for state-exchange cross-shard transactions}. 1) pre-execute, generate dependency, then exchange states; 2) divide contracts with dependency into the same shard; 3) state-exchange cross-shard transactions are ordered at the end of a certificate block;

\textbf{Applications}.

\input{shardbalance.tex}

==> shardbalance.tex <==
%\section{Adaptive Mempool Protocol}\label{sec-mempool-protocol}
\subsection{Adaptive Mempool Protocol}\label{sec-mempool-protocol}
The COE model effectively solve the data conflict problems via its deterministic global order. Recall that to establish a deterministic global order, the ordering shard need to wait for certificate blocks from \textit{all execution shards}. This works as a synchronization-ordering mechanism where each execution shard has the same block height. However, such a synchronization-ordering mechanism will lead that the performance of a sharding system is determined by the slowest execution shard. In a practical sharding system, different shards consisting of heterogeneous nodes will process transactions at various speeds. In this case, the whole system performance of the sharding system will be delayed by some slow execution shards. 

To circumvent the above issue, we present an \textit{adaptive mempool protocol}. The main idea is to allow those fast execution shards to certify multiple blocks at one consensus round while achieving a deterministic global order for them. The adaptive mempool protocol is designed as a complementary protocol that is integrated into the COE model. Figure \ref{sec-mempool-protocol} presents an overview of the adaptive mempool protocol, and we will detail it In the following.

\begin{figure}[h]
    \centering
    \includegraphics[width=3.3in]{figure/shard-balance.pdf}
    \caption{Adaptive mempool protocol}
    \label{fig:shard-balance}
\end{figure}

\noindent \textbf{Anchor blocks}. To enable an execution shard to certify multiple blocks at one consensus round, there must be one \textit{anchor block} in each execution shard at a consensus round. Specifically, when an execution shard certifies multiple blocks at a consensus round, \textit{the first certificate block} is recognized as the anchor block, e.g., $C_{j+1}^2$ in Figure \ref{sec-mempool-protocol}. An anchor block is a certificate block with the functions we discussed in \S~\ref{sec-COE-model}. It consists of a set of new cross-shard transactions, a quorum of signatures, and most importantly, a vote set for all cross-shard transactions from previous consensus rounds. The anchor blocks are used for the ordering shards to trace the heights of execution blocks in execution shards, as well as to aggregate the execution results for the two-phase commit protocol.

\noindent \textbf{Integration with the COE model}. The adaptive mempool protocol allows an execution shard to continuously create execution blocks and certify them as certificate blocks before it is aware of a new ordering block. To integrated the adaptive mempool protocol into the COE model, we need some minor modifications.

%The adaptive mempool protocol can be integrated into the COE model with minor modification. 
First, a node in an execution shard is allowed to create and certify new blocks if and only if its created anchor block has been certified (i.e., received a quorum of signatures). Furthermore, along with the three validation conditions we mentioned in \S~\ref{sec-COE-model} (\textbf{V1, V2, V3}), a node needs to check \textbf{V4:} it receives all the antecedent execution blocks and certificate blocks of a new certificate block before the node replies its signature on the new certificate block.

Second, nodes in the ordering shard need to maintain a table recording the height of the last certificate block that is committed for every execution shard. This prevents the ordering shard from picking outdated certificate blocks, i.e., blocks that have been committed. 

Third, when the ordering shard runs a consensus for execution shards, it needs to pick: i) the vote set in the anchor block $C_j^{sid}$; ii) block header of one certificate block $C_{j+n}^{sid}$; iii) all cross-shard transaction sets in blocks from block height $j$ to $(j+n)$, for an execution shard $S_E^{sid}$. 

\noindent \textit{Illustrative example:}
